NeuralFuse: Learning to Recover the Accuracy of Access-Limited Neural Network Inference in Low-Voltage Regimes

Deep neural networks (DNNs) have become ubiquitous in machine learning, but their energy consumption remains problematically high. An effective strategy for reducing such consumption is supply-voltage reduction, but if done too aggressively, it can lead to accuracy degradation. This is due to random bit-flips in static random access memory (SRAM), where model parameters are stored. To address this challenge, we have developed NeuralFuse, a novel add-on module that handles the energy-accuracy tradeoff in low-voltage regimes by learning input transformations and using them to generate error-resistant data representations, thereby protecting DNN accuracy in both nominal and low-voltage scenarios. As well as being easy to implement, NeuralFuse can be readily applied to DNNs with limited access, such cloud-based APIs that are accessed remotely or non-configurable hardware. Our experimental results demonstrate that, at a 1% bit-error rate, NeuralFuse can reduce SRAM access energy by up to 24% while recovering accuracy by up to 57%. To the best of our knowledge, this is the first approach to addressing low-voltage-induced bit errors that requires no model retraining.

==> assets/_figures/energy_accuracy_tradeoff_2.tex <==
\begin{figure}[h!t]
\includegraphics[width=\linewidth]{assets/figures_paths/IntroductionMAC_v4.pdf} 
\caption{The energy-accuracy tradeoff with 1\% bit error rate for ResNet-18 (CIFAR-10) and different NeuralFuse implementations. Bit errors are injected into model weights. The X-axis shows the percentage reduction in dynamic memory access energy for NeuralFuse implementations in a low voltage setting with 1\% bit error rate, compared to the lowest bit error-free voltage. The Y-axis shows the perturbed model accuracy with 1\% bit error rate. The circle marker area reflects the relative size of NeuralFuse to the base model.}
\end{figure}

==> assets/_tables/_table_efficience_ratio.tex <==
\begin{table}[ht]
    \centering
      \captionof{table}{The efficiency ratio ($\%$) for all NeuralFuse generators.\label{table:EffRat}}

\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{ c|c|rrrrrr }
\hline 


\multirow{2}{*}{\begin{tabular}{@{}c@{}}Base \\ Model\end{tabular}} & \multirow{2}{*}{B.E.R.} & \multicolumn{6}{c}{NeuralFuse} \\ 
& & ConvL & ConvS & DeConvL & DeConvS & UNetL & UNetS \\
\hline 

\multirow{2}{*}{ResNet18} & 1\% & 67.5 & 182 & 76.6 & 190.7 & 94.5 & 245.9 \\
 & 0.5\% & 24.7 & 73.3 & 30.7 & 62.5 & 33.6 & 88.3 \\
\hline

\multirow{2}{*}{ResNet50} & 1\% & 37.4 & 75.1 & 57.4 & 102.7 & 102.3 & 248.4 \\
 & 0.5\% & 35.2 & 108.7 & 40.4 & 92.5 & 47.4 & 124.6 \\
\hline

\multirow{2}{*}{VGG11} & 1\% & 62.3 & 212.9 & 69.5 & 165.8 & 92.0 & 251.7 \\
 & 0.5\% & 32.3 & 96.3 & 35.8 & 77.2 & 38.9 & 100.7 \\
\hline

\multirow{2}{*}{VGG16} & 1\% & 69.6 & 211.2 & 76.9 & 196.5 & 98.8 & 292.9 \\
 & 0.5\% & 30.3 & 98.1 & 33.0 & 75.3 & 40.6 & 113 \\
\hline

\multirow{2}{*}{VGG19} & 1\% & 57.6 & 147.5 & 65.5 & 141.6 & 95.4 & 250.8 \\
 & 0.5\% & 33.0 & 91.0 & 37.5 & 70.2 & 43.1 & 106.4 \\
\hline
\end{tabular}
\end{adjustbox}
\end{table}
